Z-polyregular functions

This paper introduces a robust class of functions from finite words to integers that we call Z-polyregular functions. We show that it admits natural characterizations in terms of logics, Z-rational expressions, Z-rational series and transducers. We then study two subclass membership problems. First, we show that the asymptotic growth rate of a function is computable, and corresponds to the minimal number of variables required to represent it using logical formulas. Second, we show that first-order definability of Z-polyregular functions is decidable. To show the latter, we introduce an original notion of residual transducer, and provide a semantic characterization based on aperiodicity.

==> _w <==
\section{Variable minimisation and growth rate}
\label{sec:pebblemin}

In this section, we show that the growth of the output
provides a semantic characterisation of $\Ve_k$ inside $\Ve$.
This statement is formalized in \cref{thm:skel:pebblemin},
which also provides both a decision procedure for this property
and an effective conversion algorithm.
\al{Together with a semantic separation between the different
    levels given by a suitable
    pumping lemma. A reinforcement of this pumping lemma
    will allow us to characterise aperiodicity later on.}



\al{
    Explain why this is not well expressed by the other models.
    Warning: minimising is not the same! Cite papers
    on polyregular.
}

\gd{Il faudrait qu'on dise que le résultat a déjà été formulé par
Schützenberger, mais que n'était pas formulé de manière effective (le dire subtilement).}

\begin{restatable}[Variable minimisation]{theorem}{pebbleminimisation}
	\label{thm:skel:pebblemin}
	Given $f \in \Ve$ and $k \ge 0$, we have
	$f \in \Ve_k$ if and only if \kl{$|f(w)| = \bigO(|w|^k)$}.
	Furthermore, the minimal $k$
    such that $f \in \Ve_k$ is computable,
	and the construction is effective.
\end{restatable}

This result has its own interest when understood as
a form of query optimisation. Counting the number of
valuations for a $k$-variable query is naïvely done using $k$ nested loops,
and this result concretely allows to
use the minimal amount of loops to produce the desired output.
It turns out that \cref{thm:skel:pebblemin} is 
a stepping stone towards computing the \kl{residual automaton}
of a function  $f \in \Ve$,
which is done in \cref{sec:residual}.

\begin{corollary}
    Given a $\Rel$-rational series $f$, one can decide whether $f \in \Ve$,
    compute the
    minimal $k$ such that $f \in \Ve_k$, together with
    a representation of $f$ in $\Ve_k$.
\end{corollary}

The rest of this section is devoted to the proof of  \cref{thm:skel:pebblemin}.
Let us first discuss the easy case $k=0$. Assume that $f \in \Ve$ and $|f(w)| = \bigO(1)$,
then $f(A^*)$ is finite. Moreover, for all $\delta \in \Rel$,
the language $L_{\delta} \defined \setof{w \in A^*}{f(w) = \delta}$ is regular,
thus $f = \sum_{\delta \in f(A^*)} \delta \car{L_\delta} \in \Ve_0$.
This proof scheme does not scale to functions satisfying $|f(w)| = \bigO(|w|^k)$
with $k \geq 1$, as witnessed by the map $w \mapsto |w|_a$.

To tackle the general case, we crucially rely on a \kl{quantitative pumping
lemma}. Let us first extend the $\bigO$ notation to multivariate functions
as follows.
\begin{definition}
    Let $f$ and $g$ be functions from $\Nat^n$ to $\Rat$.
    We say that $f(x_1, \dots, x_n) = \bigO(g(x_1, \dots, x_n))$ whenever
    there exists $N \in \Nat$ and $C \in \Rat$ such that
    $|f(x_1, \dots, x_n)| \leq C |g(x_1,\dots, x_n)|$ for every
    $x_1, \dots, x_n \geq N$.
\end{definition}

Let us now introduce the notion of quantitative pumping, that finds its
roots in the traditional pumping lemmas of automata theory \al{REF}.

\begin{definition}
    A function $f \colon A^* \to \Rel$ is
    \intro{$k$-pumpable} whenever for every
    $\alpha_0, \dots, \alpha_n \in A^*$,
    $u_1, \dots, u_n \in A^{\geq 1}$, 
    $|f(\alpha_0 \prod_{i = 1}^n u_i^{X_i} \alpha_i)|
    =
    \bigO(|X_1 + \cdots + X_n|^k)$.
\end{definition}

\begin{claim}
    For all $k$, for all $f \in \Ve_k$, $f$ is \kl{$k$-pumpable}.
\end{claim}

We are now ready to state the main result of this section,
from which \cref{thm:skel:pebblemin}
directly follows.
\begin{lemma}
    \label{lem:skel:pumping-lemma}
	Let $f \in \Ve$ and $k \geq 0$. The following three statements are
    equivalent:
	\begin{enumerate}
		\item \label{it:cond:class} $f \in \Ve_{k}$;
		\item \label{it:cond:growth} $|f(w)| = \bigO(|w|^{k})$;
		\item \label{it:cond:tuple}
            $f$ is \kl{$k$-pumpable}.
            %$\forall \alpha_0, u_1, \alpha_1, \dots, \alpha_{k-1}, u_k,
				  %\alpha_{k} \in A^*,
				  %|f(\alpha_0 \prod_{i = 1}^{k} (u_i)^{X_i} \alpha_i )|
				  %= \bigO(| X_1 + \cdots + X_k|^{k-1})
			  %$.
	\end{enumerate}
	Moreover this property can be decided and
	the construction is effective.
\end{lemma}

\Cref{lem:skel:pumping-lemma} is proven by induction on $k$,
and the rest of the section is devoted to proving the induction step
described hereafter.

\begin{restatable}{lemma}{skelsemanticond}
	\label{lem:skel:semantic-cond}
	Let $f \in \Ve_k$. The following three statements are equivalent:
	\begin{enumerate}
		\item \label{it:cond:class} $f \in \Ve_{k-1}$;
		\item \label{it:cond:growth} $|f(w)| = \bigO(|w|^{k-1})$;
		\item \label{it:cond:tuple}
            $f$ is \kl{$(k-1)$-pumpable}.
            %$\forall \alpha_0, u_1, \alpha_1, \dots, \alpha_{k-1}, u_k,
				  %\alpha_{k} \in A^*,
				  %|f(\alpha_0 \prod_{i = 1}^{k} (u_i)^{X_i} \alpha_i )|
				  %= \bigO(| X_1 + \cdots + X_k|^{k-1})
			  %$.
	\end{enumerate}
	Moreover this property can be decided and
	the construction is effective.
\end{restatable}

Beware that pumping properties are not easily extracted 
from the matrix presentations of \cref{sec:matrix}, as illustrated below.

\begin{example}
	Let $f(a^kb^l) = k \times l$ and $f(w) = 0$ otherwise.
	The function $f$ is $\Rel$-polyregular, of quadratic growth.
	However, $f(u w^X v)$ is at most linear for every triple $(u,v,w)$
	of words in $A^*$.
    This means that for every matrix in the generated semigroup,
    the growth is linear when iterating.
\end{example}



The key ingredient to proving \cref{lem:skel:semantic-cond} is the notion
of factorisation forests.
Given a morphism $\mu \colon A^* \to M$ into a finite monoid and
$w \in A^*$, a \kl{$\mu$-forest of $w$} with respect to $\mu$
is a word over $\hat{A} \defined A \uplus \{ \langle, \rangle \}$ that is defined
as follows.

\begin{definition}[Factorisation forest \cite{simon1990factorization}]
	Given a monoid morphism $\mu \colon A^* \to M$ and $w \in A^*$, we say that
	$F$ is a \intro{$\mu$-\emph{forest}} of $w$ when:
	\begin{itemize}
		\item either $F = a$, and $w = a \in A $;
		\item or $F = \tree{F_1} \cdots \tree{F_n}$,
		      $w = w_1 \cdots w_n$ and for all $1 \le i \le n$,
		      $F_i$ is a $\mu$-forest of $w_i \in A^+$.
		      Furthermore, if $n \ge 3$ then
		      $\mu(w_1) = \dots = \mu(w_n)$ is an idempotent of $M$.
	\end{itemize}
\end{definition}

We write $\intro*\forests{\mu}{}$ to denote the set of $\mu$-forests.
Because forests can be seen as (ordered) trees, we will use the standard vocabulary
to talk about the nodes, the sibling/parent relation, the root, the leaves
and the depth of a forest. We let $\forests{\mu}{d}$ be the set of forests
with depth at most $d$. We are interested in building functions
$\forests{\mu}{d} \fonc \Rel$ which are in $\Ve_k$. Since
the set $\forests{\mu}{d}$ is a regular language over $\hat{A}$,
we can forget about the input words which are not in $\forests{\mu}{d}$.
Let $\intro*\repword \colon \forests{\mu}{d} \to A^*$ be the function
mapping a $\mu$-forest of $w  \in A^*$ to $w$ itself.

\begin{example} \label{ex:forest} Let $M \defined (\{-1,1,0\}, \times)$.
	A forest $F\in \forests{\mu}{5}$
	(where $\mu : M^* \fonc M$ maps a word to the product of its elements)
	such that $\repword(F) = (-1)(-1)0(-1)000000$ is depicted
	in Figure~\ref{fig:ex:skel}. Double lines
	denote idempotent nodes (i.e.
	nodes with more than $3$ children).
\end{example}



When $M$ is a finite monoid, it is known that
any word in $A^*$ has a $\mu$-factorisation of
depth at most $3|M|$.

\review{if you state the bound 3|M| for Simon's factorization forest theorem, please give a reference (eg, Kufleitner MFCS 2008).}\gd{Il y a le papier de Thomas.}

This celebrated result
allows to ensure the existence of forests having
numerous idempotent nodes over large enough words.
Furthermore, this small factorisation can be computed
by a simple class of \emph{regular functions} from words to words
(see e.g. \cite{doueneau2022hiding}).
\gd{you did not explain what a regular function is. Also, the theorem is somewhat flawed because you did not define d. You could fix it before this statement, because you use it later on.}
\gd{Euh oui il faudrait dire qu'il existe $d$}

\begin{theorem}[Simon, \cite{simon1990factorization,colcombet2011green}]
	\label{thm:simon}
	Given a morphism $\mu \colon A^* \to M$ into
	a finite monoid $M$, there exists a $d$ and a 
    regular function
	$\intro*\repforest \colon A^* \to \forests{\mu}{d}$
	such that $\repword \circ \repforest$ is the identity function.

    Moreover, this construction is effective.
\end{theorem}


Following the classical connections between $\MSO$-formulas
and regular languages, we claim that for every function $f \in \Ve_k$ there exists
a monoid $M$ and a morphism $\mu \colon A^* \to M$,
such that $f(w)$ can be reconstructed using
``simple'' $\MSO$-formulas which are evaluated
along \kl{bounded-depth $\mu$-factorisations} of $w$.

\review{you should say explicitly that you fix some forest F, and emphasize the fact that the predicates between, left and right evaluate on F (and positions).}
\begin{definition}
    Let $M$ be a finite monoid, 
    $\mu \colon A^* \to M$  be a morphism,
    and $d \in \Nat$. Let us write the following $\MSO$ formulas
    over forests $F \in \forests{\mu}{d}$ that factorise a word $w$:
    \begin{itemize}
        \item $\intro*\msoprod_m(x,y)$
            evaluates to $\top$ if and only if
            $x \leq y$ and $\mu(w[x] \dots w[y]) = m$
            where $w \defined \repword(F)$
        \item $\intro*\msoleft_m(x)$ that evaluates to $\top$
if and only if $\mu(w[1] \dots w[x]) = m$
            \item $\intro*\msoright_m(x)$ that evaluates to $\top$
if and only if $\mu(w[x] \dots w[|w|]) = m$
\item $\intro*\msoisleaf(x)$ for the predicate asserting that $x$
is a leaf in the forest $F$.
    \end{itemize}
\end{definition}

We will be interested in a simple fragment $\intro*\INV$ of $\MSO$ over $\forests{\mu}{d}$
obtained by restricting formulas to quantifier free formulas
using only the predicates $\msoprod_m$, $\msoleft_m$, and $\msoright_m$ where
$m$ ranges over $M$, and where every free variable $x$
is guarded by the predicate $\msoisleaf(x)$.

\begin{lemma}
	\label{lem:skel:to-forest}
	For all $f \in \Ve_k$, one can build
	a finite monoid $M$, a depth $d \in \Nat$,
	a surjective morphism $\mu \colon A^* \to M$,
	constants $\delta_i \in \Rel$,
	formulas $\psi_i(x_1, \dots, x_k) \in \INV$,
	such that
	for every word $w \in A^*$,
	for every \kl{factorisation forest} $F \in \forests{\mu}{d}$ of $w$,
	$f(w) = \sum_{i = 1}^{n} \delta_i \times \card{\psi_i}(F)$.
\end{lemma}

In the rest of this section, we therefore
focus on the number of free variables in $\Rel$-linear combinations
of $\card \psi$ where $\psi \in \INV$.
The crucial idea is that one can leverage the structure of the forest
$F \in \forests{\mu}{d}$
to compute $\card \psi$ more efficiently, at the cost of
building a non-$\INV$ formula.
The idea will be to compute the value of entire subtrees of the
factorisation forest at once.

For that, we explore the structure of the forest $F$
as follows: given a node $t$ in a forest $F$, we define its
skeleton to be the subforest rooted at that node, containing
only the right-most and left-most children recursively.
This notion was already introduced
in \cite{doueneau2022hiding} for the study of \kl{$\Nat$-polyregular functions}.

\begin{definition} Let $F \in \forests{\mu}{}$ and $\nod \in \Nodes(F)$, we define
	the \intro{skeleton} of $\nod$ by:
	\begin{itemize}
		\item if $\nod = a\in A$ is a leaf, then $\intro*\Ske(\nod) \defined \{ \nod \}$;
		\item otherwise if $\nod = \tree{F_1} \cdots \tree{F_n}$, then
		      $\Ske(\nod) \defined \{\nod\} \cup \Ske(F_1) \cup \Ske(F_n)$.
	\end{itemize}
\end{definition}

Given a word $w$, a $\mu$-factorisation $F$ of $w$, and a node
$\nod \in \Nodes(F)$, the set of nodes $\Ske(\nod)$ defines
a $\mu$-factorisation of a (scattered) subword $u$ of $w$: the one
obtained by concatenating the leaves of $F$ that are in $\Ske(\nod)$.
See \cref{fig:ex:skel} for an example of a skeleton.
A crucial property of $\Ske(\nod)$ seen as a forest is that
$\mu(\repword(\Ske(\nod))) = \mu(F')$ where $F'$ is the subforest
of $F$ rooted at $\nod$, because we only remove inner idempotent
nodes.


\begin{figure}[h!]
	\newcommand{\couleur}{blue!70}
	\centering
    \resizebox{\linewidth}{!}{
	\begin{tikzpicture}[
			skel/.style={
					circle, fill=blue,
					inner sep=2pt,
					minimum width=1pt,
				}
		]


		\newcommand{\texte}{\small \bfseries \sffamily \mathversion{bold} }

		% Input 1
		\node[above] at  (0,0)  {$-1$};
		\node[above] at  (1,0)  {$-1$};
		\node[above] at  (2,0)  {$0$};
		\node[above] at  (3,0)  {$-1$};
		\node[above] at  (4,0)  {$0$};
		\node[above] at  (5,0)  {$0$};
		\node[above] at  (6,0)  {$0$};
		\node[above] at  (7,0)  {$0$};
		\node[above] at  (8,0)  {$0$};
		\node[above] at  (9,0)  {$0$};

		\draw[double] (4,0.975) -- (8,0.975);
		\draw[] (3,1.5) -- (6,1.5);
		\draw[double] (2,1.975) -- (9,1.975);
		\draw[] (0,2) -- (1,2);
		\draw[] (0.5,2.5) -- (6.5,2.5);

		\draw[] (0,2) -- (0,0.5);
		\draw[] (1,2) -- (1,0.5);
		\draw[] (0.5,2) -- (0.5,2.5);

		\draw[] (2,2) -- (2,0.5);
		\draw[] (9,2) -- (9,0.5);

		\draw[] (6.5,2) -- (6.5,2.5);
		\draw[] (3.5,2.5) -- (3.5,2.75);

		\draw[] (3,1.5) -- (3,0.5);
		\draw[] (4,1) -- (4,0.5);
		\draw[] (5,1) -- (5,0.5);
		\draw[] (6,1.5) -- (6,0.5);
		\draw[] (7,1) -- (7,0.5);
		\draw[] (8,1) -- (8,0.5);

		\draw[] (4.5,2) -- (4.5,1.5);

		\node[skel] at (4.5,1.5) {};
		\node[skel] at (6,1) {};
		\node[skel] at (3,0.5) {};
		\node[skel] at (4,0.5) {};
		\node[skel] at (8,0.5) {};


	\end{tikzpicture}
}

	\caption{\label{fig:ex:skel}  A forest $F$ with $\repword(F) = (-1)(-1)0(-1)000000$
		together with a skeleton in blue.}
\end{figure}

\review{Please introduce Claim 4.8. The reader does not know where you are going.}
\gd{J'ai refait cette formalisation  des origines dans  le nouveau papier "last pebble transducers",
on peut peut-être s'en re-servir (ainsi que des dessins).}

To a given leaf $a$ of a forest $F$ one can associate a node $\nod$
such that $a \in \Ske(\nod)$. Several nodes $\nod$ can be associated
to the same leaf $a$, but as claimed below, there always
exists a maximal node $\nod$ corresponding to $a$. This allows to partition
leaves according to their \emph{skeleton-root}.

\begin{claim}
	\label{claim:skel:skeletons-totally-ordered}
	Let $x \in \Leaves(F)$, there exists $\nod \in \Nodes(F)$ such that
	$x \in \Ske(\nod)$. Furthermore, if $\nod'$ is such
	that $x \in \Ske(\nod')$, then $\Ske(\nod) \subseteq \Ske(\nod')$ or
	$\Ske(\nod') \subseteq \Ske(\nod)$.
\end{claim}

It follows from \cref{claim:skel:skeletons-totally-ordered}
that the set $\Leaves(F)$ can be partitioned depending
on the maximal skeleton (for inclusion) which contains a leaf.

\begin{definition}[Skeleton of a leaf]
	Let $\intro*\partitionskel \colon \Leaves(F) \to \Nodes(F)$
	map a leaf $x$ to the $\nod \in \Nodes(F)$ such that $x \in \Ske(\nod)$
	and $\Ske(\nod)$ is maximal for inclusion.
\end{definition}


Skeletons enable us to introduce a notion of dependency
for leaves, inspired by  \cite{doueneau2022hiding}.


\begin{definition}[Observation]
	We say that $\nod' \in \Nodes(F)$ \intro{observes} $\nod \in \Nodes(F)$
	if either $\nod'$ is an ancestor of $\nod$, or the immediate
	left or right sibling of an ancestor of
	$\nod$, or an immediate sibling of $\nod$,
	or $\nod' = \nod$.
\end{definition}

\begin{definition}[Dependent leaves]
	In a forest $F$, a leaf $y$ \intro{depends} on a leaf $x$
	when $\partitionskel(y)$ \kl{observes} $\partitionskel(x)$.
\end{definition}

Beware that this relation $x \intro*\dependson y$
is not symmetric. This allows us to ensure that the number of
leaves $y$ that depend on a fixed leaf $x$ is uniformly bounded.
\begin{claim}
	\label{rem:skel:bound-depnodes}
	Given $d \ge 0$, there exists a (computable) bound $N_d \in \Nat$
	such that for every $F \in \forests{\mu}{d}$
	and every leaf $x \in \Leaves(F)$, there exist at most
	$N_d$ leaves which \kl{depend} on $x$.
\end{claim}

It is a routine check that for every fixed $d$,
one can define the predicate
$\msodep(x,y)$ in $\MSO$ over $\forests{\mu}{d}$ checking whether
$x$ depends on $y$ or $y$ depends on $x$, i.e., the \emph{symmetrised}
version of $x \dependson y$.
We generalize this predicate to tuples $\vec{x} \defined (x_1, \dots, x_k)$
via:
\begin{equation*}
	\intro*\msodep(\vec{x}) \defined \left\{
	\begin{array}{ll}
		\top                                                  & \mbox{for } k=0;  \\
		\top  \mbox{ if and only if } x_1 \mbox{ is the root} & \mbox{for } k=1 ; \\
		\bigvee_{i \neq j} \msodep(x_i,x_j)                   & \mbox{otherwise.}
	\end{array}
	\right.
\end{equation*}
Notice that the independence (or dependence) of a tuple of leaves
$\vec{x}$ only depends on the tuple $\partitionskel(x_1),
	\dots, \partitionskel(x_n)$.
The notion of dependent leaves is motivated by the fact
that counting dependent leaves can be done one variable less,
as shown in \cref{lem:skel:inv-decomp}.

\begin{lemma}
	\label{lem:skel:inv-decomp}
	Let $d \ge 0$, $k \geq 1$, and let $\psi(x_1, \dots, x_k)$ be an
	$\MSO$ formula over $\forests{\mu}{d}$, then
	$\card (\psi(\vec{x}) \wedge \msodep(\vec{x}))  : \forests{\mu}{d} \fonc \Rel$
	effectively belongs to $\Ve_{k-1}$.
\end{lemma}

%\gd{Quel est l'intérêt de ce corollaire en fait?}

%\begin{corollary}
%\label{cor:skel:dep-growth-rate}
%Let $f = \sum_{i = 1}^{n} z_i \card{(\psi_i \wedge \msodep)}$
%where each $\psi_i$ has $k$ free variables.
%Then $f \in \Ve_{k-1}$ over $\forests{\mu}{d}$
%and in particular
%$|f(F)| = \bigO(|F|^{k-1})$.
%\end{corollary}


Now, let $f \in \Ve_k$ verifying \cref{skelsemanticond}
in \cref{lem:skel:lemmapoly}. \review{Pas le bon lemme.}
\revv{There is no item 3 in Lemma 4.17. Did you mean 4.2?}
Thanks to \cref{lem:skel:to-forest}
and \cref{thm:simon}, there exists $\mu : A^* \fonc M$, $d \ge 0$, $\delta_i \in \Rel$,
$\psi_i(x_1, \dots, x_k) \in \INV$ such that:
\begin{equation}
	\label{eq:findep}
	\begin{aligned}
		f & = \left(\sum_{i=1}^n \delta_i \card \psi_i \right) \circ \repforest               \\
		  & = \underbrace{\left(\sum_{i=1}^n \delta_i \card (\psi_i \wedge \msodep) \right)}_ %
		{\defined \intro*\fdep} \circ \repforest
        \\
          &+
		\underbrace{\left(\sum_{i=1}^n \delta_i \card (\psi_i \wedge \neg\msodep) \right)}_%
		{\defined \intro*\findep} \circ \repforest                                            \\
	\end{aligned}
\end{equation}
Using \cref{lem:skel:inv-decomp}, $\fdep \in \Ve_{k-1}$.
Since $\Rel$-polyregular functions are closed under pre-composition
by a regular function (it is a consequence of \cref{prop:polypoly}),
it suffices to prove that $\findep = 0$ to conclude that $f \in \Ve_{k-1}$.
\review{Don't you need the stability by composition with a regular function to preserve membership in $P_k$ and not just in P?} \gd{oui}
%
%\gd{todo: Al: INLINER LE COR
%	\begin{corollary}
%		\label{rem:preli:precomp-regular}
%		The class $\Ve$ is closed under pre-composition with a
%		polyregular function, and the class $\Ve_k$
%		is closed under pre-composition with a regular function.
%	\end{corollary}}
%
Assuming that $\findep \neq 0$, we are going to build a
``pumping family'' of input forests so that $\findep$ exhibits
an asymptotic behavior of $\Omega(|F|^{k})$, which is a
contradiction.  \review{explain that this is because of Item 3 in Lemma 4.2.}
 For that, let us
define how we are going to pump words.

\begin{definition}[Pumping family]
	A $(\mu, d)$-\intro{pumping family} of size $k \geq 1$ is given by
	words $\alpha_0, u_1, \alpha_2, \dots, \alpha_{k-1}, u_k, \alpha_k \in
    A^*$,
    such that $u_i \neq \varepsilon$.
	Given $\bar{X} = X_1, \dots, X_k \ge 0$ the family provides
	the word $w^{\bar{X}} \defined \alpha_0 \prod_{i = 1}^{k} (u_i)^{X_i} \alpha_i$
	together with a \kl{$\mu$-factorisation} $F^{\bar{X}}$ of $w^{\bar{X}}$ of depth at most $d$.
\end{definition}
\begin{remark}
	A $(\mu,d)$-\kl{pumping family} of size $k$ satisfies that
	$|w^{\bar{X}}| = \Theta(X_1 + \dots + X_k)$,
	and $|F^{\bar{X}}| = \Theta(X_1 + \dots + X_k)$
	since its depth is bounded by $d$.
\end{remark}



\begin{lemma}
	\label{lem:skel:indep-iter-zero}
	Let $\findep$ be defined as in \cref{eq:findep}.
	If $\findep \neq 0$, there exists a $(\mu,d)$-\kl{pumping family} of size $k$
	such that $f(F^{\bar{X}})$ is asymptotically
	a $\Rel$-polynomial in $X_1, \dots, X_k$
	with a non-zero coefficient for $X_1 \cdots X_k$.
	Moreover, one can decide whether $\findep = 0$.
\end{lemma}


Now, we are almost ready to conclude the proof of \cref{lem:skel:semantic-cond}.
The only difficulty left is
handled by the following technical lemma which enables
to lift a bound on the asymptotic growth of polynomials
to a bound on their respective degrees. It is also
reused in \cref{sec:aperiodic}.

\begin{lemma}[Bounding polynomials]
	\label{lem:skel:lemmapoly}
	Let $P,Q \in \mathbb{R}[X_1, \dots, X_n]$,
	$C, N_0 \ge  0$,
	be such that
	for all $x_1, \dots, x_n \in \mathbb{N}_{\geq N_0}$,
	$|P(x_1, \dots, x_n)| \leq C | Q(x_1, \dots, x_n)|$.
	Then $\deg (P) \leq \deg (Q)$.
\end{lemma}
\begin{proof}[Proof of \cref{lem:skel:semantic-cond}]
	The only non-trivial implication is
	\cref{it:cond:tuple} $\implies$ \cref{it:cond:class}.
	Let $f \in \Ve_k$ verifying the conditions of \cref{it:cond:tuple}.
	We can decompose this function following \cref{eq:findep}.
	As observed above, we only need to show that
	$\findep = 0$.

	Consider a \kl{pumping family}
	$(w^{\bar{X}}, F^{\bar{X}})$
	of size $k$,
	we have:
	\begin{equation*}
		|\findep(F^{\bar{X}})| %= |(f' - \fdep)(F^{\bar{X}})|
		= |f(w^{\bar{X}}) - \fdep(F^{\bar{X}})|
		= \bigO(|X_1 + \dots + X_k|^{k-1}).
	\end{equation*}
	Assume by contradiction that $\findep \neq 0$,
	\review{Lemma 4.16} provides us with
	a \kl{pumping family} such that
	$\findep(F^{\bar{X}})$ is asymptotically a polynomial
	with non-zero coefficient for $X_1 \dots X_k$, in particular,
	it is of degree greater than $k$. However,
	this polynomial is bounded asymptotically by $(X_1 + \dots + X_k)^{k-1}$,
	hence \cref{lem:skel:lemmapoly} yields a contradiction.


	The construction of $\repforest$, $\fdep$, and $\findep$ are effective,
	therefore so is our procedure. Moreover, one can decide
	whether $\findep = 0$ thanks to \cref{lem:skel:indep-iter-zero}.
\end{proof}





==> parts/fig-run-H-transducer.tex <==
\begin{figure}[h!]

\centering
\begin{tikzpicture}{scale=1}

	\newcommand{\coulun}{red}
	\newcommand{\coulde}{blue}


	% Input 2

	
	\draw  (7,1.7) -- (0,1.7) -- (0,2.2) -- (7,2.2) --  (7,1.7);
	

	\node[above] at (0.5,1.75) {$a$};
	\draw[dotted] (1,2.3) -- (1,-2.7);
	\node[above] at (1.5,1.75) {$a$};
	\draw[dotted] (2,2.3) -- (2,-2.7);
	\node[above] at (2.5,1.75) {$b$};
	\draw[dotted] (3,2.3) -- (3,-2.7);
	\node[above] at (3.5,1.75) {$a$};
	\draw[dotted] (4,2.3) -- (4,-2.7);
	\node[above] at (4.5,1.75) {$b$};
	\draw[dotted] (5,2.3) -- (5,-2.7);
	\node[above] at (5.5,1.75) {$b$};
	\draw[dotted] (6,2.3) -- (6,-2.7);
	\node[above] at (6.5,1.75) {$b$};
	

	% Run
	\draw[->,thick,color=\coulun](0,1.3) -- (1,1.3);
	\draw[->,thick,color=\coulun](1,1.3) -- (2,1.3);
	\draw[->,thick,color=\coulun](2,1.3) -- (3,1.3);
	\draw[->,thick,color=\coulun](3,1.3) -- (4,1.3);
	\draw[->,thick,color=\coulun](4,1.3) -- (5,1.3);
	\draw[->,thick,color=\coulun](5,1.3) -- (6,1.3);
	\draw[->,thick,color=\coulun](6,1.3) -- (7,1.3);
	\draw[-,thick,color=\coulun](0,1.4) -- (0,1.2);
	\node[above,color=\coulun] at (0.2,1.25) {\small $q_0$};
%	\draw[-,thick](1,1.4) -- (1,1.2);
	\node[above,color=\coulun] at (1.2,1.25) {\small $q_1$};
%	\draw[-,thick](2,1.4) -- (2,1.2);
	\node[above,color=\coulun] at (2.2,1.25) {\small $q_2$};
%	\draw[-,thick](3,1.4) -- (3,1.2);
	\node[above,color=\coulun] at (3.2,1.25) {\small $q_3$};
%	\draw[-,thick](4,1.4) -- (4,1.2);
	\node[above,color=\coulun] at (4.2,1.25) {\small $q_4$};
%	\draw[-,thick](5,1.4) -- (5,1.2);
	\node[above,color=\coulun] at (5.2,1.25) {\small $q_5$};
%	\draw[-,thick](6,1.4) -- (6,1.2);
	\node[above,color=\coulun] at (6.2,1.25) {\small $q_6$};
%	\draw[-,thick](7,1.4) -- (7,1.25);
	\node[above,color=\coulun] at (7.2,1.25) {\small $q_7$};
	
%	\draw[->,thick,color=\coulde](6,1.3) -- (7,1.3);
	\node[above,color=\coulde] at (7.35,0.9) {\small $F(q_7)$};
	\draw[-,thick, color=\coulde](6.9,1) -- (7,1);
	\node[above,color=\coulde] at (6.5,0.4) {\small $\lambda(q_6,b)(\movi)$};
	\draw[-,thick, color=\coulde](6,0.5) -- (7,0.5);
	\node[above,color=\coulde] at (6,-0.1) {\small $\lambda(q_5,b)(b)$};
	\draw[-,thick, color=\coulde](5,0) -- (7,0);
	\node[above,color=\coulde] at (5.5,-0.6) {\small $\lambda(q_4,b)(bb)$};
	\draw[-,thick, color=\coulde](4,-0.5) -- (7,-0.5);
	\node[above,color=\coulde] at (5,-1.1) {\small $\lambda(q_3,a)(bbb)$};
	\draw[-,thick, color=\coulde](3,-1) -- (7,-1);
	\node[above,color=\coulde] at (4.5,-1.6) {\small $\lambda(q_2,b)(abbb)$};
	\draw[-,thick, color=\coulde](2,-1.5) -- (7,-1.5);
	\node[above,color=\coulde] at (4,-2.1) {\small $\lambda(q_1,a)(babbb)$};
	\draw[-,thick, color=\coulde](1,-2) -- (7,-2);
	\node[above,color=\coulde] at (3.5,-2.6) {\small $\lambda(q_0,a)(ababbb)$};
	\draw[-,thick, color=\coulde](0,-2.5) -- (7,-2.5);
	

	
\end{tikzpicture}

\caption{\label{fig:shape-run-H} Behavior of a $\Oras$-transducer
on input $aababbb \in A^*$.}

\end{figure}


==> parts/trash.tex <==


\section{Trash: syntactic morphisms and decompositions}

%
%\begin{definition}[Variety] A \emph{variety} is a
%class of finite monoids which is closed under cartesian products
%and \gd{divisions, but we do not use it for the moment}.
%\end{definition}
%

\begin{definition}[Decomposition] Let $\Oras \subseteq A^* \fonc \Rel$.
Let $f : A^* \fonc \Rel$, $\mu : A^* \fonc M$ be a
morphism into a finite monoid
and $(h_m)_{m \in M}$ be a family of functions of $\Oras$.
We say that $(M, \mu, (h_m)_{m})$
is an \emph{$\Oras$-decomposition} of $f$ if
$\displaystyle f = \sum_{m \in M} \car{m} \cauchy h_m$
where $\car{m} : u \mapsto \mathbf{1}_{\mu(u) = m}$.
\end{definition}
%


\begin{claim}  Let $\Oras$ be a submodule 
of $A^* \fonc \Rel$. The set of functions of
$A^* \fonc \Rel$ which have an $\Oras$-decomposition
is a submodule of $A^* \fonc \Rel$. Furthermore, the decompositions
for sum and scalar product can effectively be built.
\end{claim}

\begin{proof} Let $f,g : A^* \fonc \Rel$ and $(M, \mu, (h_m)_m)$
(resp. $(N, \nu, (h_n)_n)$) be an $\Oras$-decomposition
of $f$ (resp. of $g$). Let  $\alpha \in \Rel$. Then $(M, \mu, (\alpha h_m)_m)$
is an $\Oras$-decomposition of $\alpha f$ and
$(M \times N, \mu \times \nu, (h_{(m,n)})_{(m,n) \in M \times N})$.
is an $\Oras$-decomposition of $f+g$.
\end{proof}


%Given a variety $\Var$, we define by induction on $k \ge {-}1$
%the submodule $\Level{k}{\Var} \subseteq A^* \fonc \Rel$ as follows.
%For $k = -1$, $\Level{-1}{\Var}$ is the set of constant functions.
%Otherwise $\Level{k}{\Var}$ is the submodule of
%functions which have an $\Level{k-1}{\Var}$-decomposition.
%We let $\Level{}{\Var} \defined \bigcup_{k} \Level{k}{\Var}$.
%
%Let $\Monos$ be the class of all monoids.

\begin{lemma} \label{lem:equi} For all $k \ge 1$, $f \in \Ve_k$
if and only if it has a $\Ve_{k-1}$-decomposition.
Furthermore, the transformations are effective.
\end{lemma}

\begin{proof} \gd{Voir la preuve d'Al au dessus.}
\end{proof}

We say that a decomposition is \emph{aperiodic} if 
the monoid $M$ is aperiodic.

\begin{lemma} For all $k \ge 1$, $f \in \We_k$
if and only if it has an aperiodic $\We_{k-1}$-decomposition.
Furthermore, the transformations are effective.
\end{lemma}


We now introduce the notion of \emph{syntactic decomposition}.

\begin{definition} Given $f \in \Ve_k$, we define
its $k$-syntactic congruence $\equiv_f$ by $u \equiv_f u'$
if and only if for all $\alpha, \beta \in A^*$,
$(\push{f}{\alpha u}) \polysim{k-1} (\push{f}{\alpha u'})$.
\end{definition}
%
In particular for $k=0$, we have $u \equiv_f u'$ if and only if
for all $\alpha, \beta \in A^*$, $ f(\alpha u \beta) = f(\alpha u' \beta)$
(indeed, $\Ve_{-1} = \{0\}$).
If $f$ was the indicator function of a regular language $L$, 
then $\equiv_f$ is exactly the syntactic congruence of
the language $L$.

\begin{lemma} For $k \ge 0$, $f \in \Ve_k$, $\equiv_f$ is a congruence of finite index.
\end{lemma}

\begin{proof} It is clearly an equivalence relation.
If  $u \equiv_f u'$ and $v \equiv_f v'$, then
for all $\alpha \in A^*$ we have
$(\push{f}{\alpha u}) \polysim{k-1} (\push{f}{\alpha u'})$
and therefore $(\push{f}{\alpha uv}) =  (\push{(\push{f}{\alpha u})}{v})
\polysim{k-1} (\push{(\push{f}{\alpha u'})}{v}) = (\push{f}{\alpha u'v})$.
Furthermore, $(\push{f}{\alpha u'v}) \polysim{k-1} (\push{f}{\alpha u' v'})$
and thus $uv \equiv_f u'v'$.

Now, let us show that it has finite index.
Let us assume that $k \ge 1$. By Lemma~\ref{lem:equi},
$f$ has a $\Ve_{k-1}$-decomposition $(M, \mu, (h_m)_m)$.
We claim that if $\mu(u) = \mu(u')$, then $u \equiv_f u'$.
Indeed, given $\alpha \in A^*$ we have:
\begin{equation*}
\begin{aligned}
\push{f}{\alpha u}
&= \sum_{m \in M} \push{(\chi_m \cauchy h_m)}{\alpha u}\\
&\polysim{k-1} \sum_{m \in M} (\push{\chi_m}{\alpha u}) \cauchy h_m
\text{~~\gd{by the above remark of Al}}\\
&= \sum_{m \in M} (\push{\chi_m}{\alpha u'}) \cauchy h_m\\
&\polysim{k-1} \sum_{m \in M} \push{(\chi_m \cauchy h_m)}{\alpha u'}
\text{~~\gd{by the above remark of Al}}\\
&= \push{f}{\alpha u'}\\
\end{aligned}
\end{equation*}
\gd{the case of $k=0$ has to be treated separately}.
\end{proof}


\begin{definition} The $k$-syntactic morphism of $f \in \Ve_k$ is the
function $\mu_f : A^* \fonc A^* / \equiv_f$ which maps $u$
to its equivalence class of $u$ for the $k$-residual congruence $\equiv_f$.
\end{definition}


\begin{definition}[$k$-syntactic decomposition]
We say that a $\Ve_{k-1}$-decomposition $(M, \mu, (h_m)_m)$
of $f \in \Ve_k$ is \emph{$k$-syntactic}
if the following holds: 
\begin{itemize}
\item $\mu$ is the $k$-syntactic morphism of $f$;
\item for all $m \in M$, $h_m \in \Vect{\Rel}(\Res(f))$.
\end{itemize}
\end{definition}


\begin{lemma} Given $f \in \Ve_k$, one can build
a $k$-syntactic $\Ve_{k-1}$-decomposition of $f$.
\end{lemma}

\begin{proof}

\end{proof}



\begin{theorem} \label{theo:poly-growth}
The class of $\Rel$-polyregular functions is exactly
the class of $\Rel$-rational series which have polynomial growth.
\end{theorem}



\begin{definition} Let $f \colon A^* \fonc \Rel$. We say that
$(I, \mu, F)$ is a \emph{$\Rel$-representation} of $f$
if there exists $n \ge 0$ such that $I \in \Rel^n$,
$F \in \Rel^n$, $\mu \colon A^* \fonc \Rel^{n \times n}$ is a
monoid morphism, and for all $u \in A^*$,
$f(u) = I \mu(u) {}^{t} F$.
\end{definition}
%
It known that $\Rel$-rational series of polynomial growth have
a specific representation. \gd{Mais ce résultat ne semble pas effectif,
la preuve fait des Q-modules bizarres, sinon on n'aurait pas besoin des forêts hehe.}

%\begin{theorem}[{\cite[Corollary 2.4 p. 159]{berstel2011noncommutative}}]
%One can decide if a $\Rel$-rational series $f:A^* \fonc \Rel$ has polynomial growth.
%\end{theorem}


\begin{theorem}[{\cite[Theorem 2.5 p. 159]{berstel2011noncommutative}} \cite{schutzenberger1962}]
\label{theo:schutz}
Let  $f \colon A^* \fonc \Rel$ be a $\Rel$-rational series
such that $|f(u)| = \bigO(|u|^k)$.
Then $f$ has a $\Rel$-representation $(I, \mu, F)$ where $\mu \colon A^* \fonc \Rel^{n \times n}$
is of the upper triangular form:
\begin{equation}
\begin{aligned}
\begin{pmatrix} 
\mu_0 & \star & \cdots & \star \\ 
0 & \mu_1 & \cdots & \star \\ 
\vdots & \vdots & \ddots & \vdots \\ 
0 & 0 & \cdots & \mu_k
\end{pmatrix}
\end{aligned}
\end{equation}
where the $\mu_i : A^* \fonc \Rel^{n_i \times n_i}$
are morphisms such that $\mu_i(A^*)$ is finite.
\end{theorem}

%\begin{remark} Each $\mu_i(A^*)$ is finite has something
%to do with the bounded copies of SSTs.
%\end{remark}

\begin{lemma} Let $f$ be a $\Rel$-rational series such that \gd{},
then $\Res(f) / \polysim{k-1}$ is finite.
\end{lemma}

\begin{proof}
$f_u(v) = I \mu(u) \mu(v) F \polysim{k-1} (I \mu(u))[n+1]$ \gd{haut-droite de $\mu(v)$}  $F[0]$
\gd{sauf que $(I \mu(u))[n+1]$ ne peut prendre qu'un nombre fini de valeurs,
par hypothèse}.
\end{proof}

Now, let us show by induction on $k \ge 0$ that if $f$ is a $\Rel$-rational
series such that $|f(u)| = \bigO(|u|^k)$, then there exists
a $\Ve_k$-transducer which computes $f$.
For $k = 0$, we note by Theorem~\ref{theo:schutz}
that $f^{-1}(k)$ is a regular language for all $k \in \Rel$.
If $k \ge 1$, 
\gd{On fait la construction du $k$-automate des résiduels,
et ça marche.}



==> tikz/classes-inclusion.tex <==
\begin{tikzpicture}[
    desc/.style={
        draw=black,
        text centered, rounded corners, minimum height=4em,
        execute at begin node={\begin{varwidth}{0.3\linewidth}},
        execute at end node={\end{varwidth}}
    },
    sect/.style={
        midway,
        above,
        execute at begin node={\tiny \begin{varwidth}{0.2\linewidth}},
        execute at end node={\end{varwidth}}
    },
    equiv/.style={
        thick
    }
]
    \node[desc] (CMSO) at (0,0) {$\card \MSO$ formulas};
    \node[desc] (PEB) at (-2,-2) {Pebble transudcers with $\Rel$ output};
    \node[desc] (REXP) at (2,-2) {$\Rel$-rational series with polynomial growth};

    \draw[equiv] (CMSO.west) edge[in=90,out=180] 
        node[sect, left] {\cref{sec:pebble}}
                (PEB);
    \draw[equiv] (CMSO.east) edge[in=90,out=0] 
        node[sect, right] {\cref{sec:matrix} \\and \cref{sec:series}}
        (REXP);
\end{tikzpicture}


